ManiPose: A Comprehensive Benchmark for Pose-aware Object Manipulation in Robotics

Robotic manipulation in everyday scenarios, especially in unstructured environments, requires skills in pose-aware object manipulation (POM), which adapts robots' grasping and handling according to an object's 6D pose. Recognizing an object's position and orientation is crucial for effective manipulation. For example, if a mug is lying on its side, it's more effective to grasp it by the rim rather than the handle. Despite its importance, research in POM skills remains limited, because learning manipulation skills requires pose-varying simulation environments and datasets. This paper introduces ManiPose, a pioneering benchmark designed to advance the study of pose-varying manipulation tasks. ManiPose encompasses: 1) Simulation environments for POM feature tasks ranging from 6D pose-specific pick-and-place of single objects to cluttered scenes, further including interactions with articulated objects. 2) A comprehensive dataset featuring geometrically consistent and manipulation-oriented 6D pose labels for 2936 real-world scanned rigid objects and 100 articulated objects across 59 categories. 3) A baseline for POM, leveraging the inferencing abilities of LLM (e.g., ChatGPT) to analyze the relationship between 6D pose and task-specific requirements, offers enhanced pose-aware grasp prediction and motion planning capabilities. Our benchmark demonstrates notable advancements in pose estimation, pose-aware manipulation, and real-robot skill transfer, setting new standards for POM research. We will open-source the ManiPose benchmark with the final version paper, inviting the community to engage with our resources, available at our website:https://sites.google.com/view/manipose.

==> archive/pose_old.tex <==
% In POM, it's crucial to observe object poses to provide relevant knowledge for downstream operations and decision-making. Therefore, we need to train a pose estimation module to estimate object poses. This process requires a rich dataset with annotated poses. Several datasets have been released, achieving high prediction accuracy within these collections. However, current datasets face two main problems: 1) The amount of data is insufficient, and the available data are scattered, limiting the generalizability of pose estimation. 2) The pose annotations in the data are not aligned, being marked through manual rules, which hampers large-scale expansion.

% Addressing these issues, this paper introduces a new General Object Pose Dataset. This dataset incorporates objects from various datasets, classifying them based on their type, geometric shape, and function, and marks them according to a consistent pose annotation standard. This approach enhances the dataset's generalizability and expandability. The following sections detail the dataset and pose annotation.



==> archive/related_old.tex <==
% The realm of robot manipulation benchmarks is diverse, encompassing a wide array of object types and task complexities. These benchmarks have provided rich environments that include interactions with rigid bodies, articulated bodies, and soft bodies, along with complex tasks such as grasping, trajectory planning, and high precision operations. They are instrumental in offering efficient physical simulation and rendering capabilities, supporting a multitude of baseline approaches for decision-making and planning, including imitation learning, reinforcement learning (RL), and sampled-based planning strategies. Prominent environments like Sapien and ManiSkill2 are noted for their exceptional simulation quality and task variety. Despite these advancements, the specific challenges posed by the variability of object poses in real-world scenarios remain largely unaddressed. Most benchmarks do not consider how the changing poses of objects can complicate manipulation tasks, lacking tasks designed to test the adaptability of manipulation strategies to pose variations. The ManiPose benchmark proposed in this paper aims to fill this gap by providing a novel environment tailored for the evaluation of pose-aware manipulation strategies. It introduces manipulation scenarios sensitive to object poses, incorporating diverse objects and complex task settings that reflect the intricacies of real-world object manipulation.


% The challenge of object pose estimation has been a significant focus of research for many years, evolving from early methods reliant on multi-view 2D imagery and 3D reconstruction to recent advancements in 3D pose estimation leveraging neural network capabilities. Initially, pose estimation efforts were hindered by issues such as occlusions and the variability in image quality and lighting. However, the increased processing power for handling 3D point clouds has led to the development of more accurate pose estimation methods. Despite these technological advances, the field is still constrained by a lack of sufficient annotated pose data and inconsistencies in pose definitions across different datasets, which limit the generalization capabilities of pose estimation techniques. This paper addresses these challenges by introducing a large-scale object pose dataset along with a baseline method for pose estimation. By standardizing data annotation formats and testing the effectiveness of pose estimation networks, this contribution aims to enhance the applicability and generalization of pose-informed manipulation strategies, paving the way for more robust and adaptable robotic manipulation capabilities.

==> text/introduction.tex <==
\section{introduction}
With the steady progression of artificial intelligence and the advent of foundation models, the development of embodied AI has seen a remarkable acceleration. Impressively, robots are now equipped with the skills to perform kitchen duties, such as inserting a lasagna into an oven, setting a pot on the stove, placing a plate inside a microwave, hanging a mug on a rack, or storing a cup on a shelf. The ability to recognize and precisely adjust the 6D pose of objects for specific tasks is crucial for robots operating in human environments. The concept of 6D pose stands as a fundamental primitive in tasks related to grasping, manipulation, and planning, highlighting the advanced capabilities and practical utility of these robotic systems.


Pose estimation is a critical component for a wide variety of computer vision and robotic tasks.

For motion planning and control, estimating an object’s pose can help a robot avoid collisions or plan how to use the object for a given task.  

Task-specific plan ~\cite{TAX-Pose}, relative placement tasks, move object A so that it will be in the “goal pose". 



Overall, our contributions are summarized as follows: 

\begin{itemize}
    \item The unification of 6D pose definitions across multiple rigid body datasets, YCB~\cite{calli2015ycb}, OmniObject3D~\cite{wu2023omniobject3d}, PACE~\cite{you2023pace}, where the X-axis represents the forward direction of the object, and the Y-axis defines the direction in which the object can be grasped perpendicularly. And PartNet-Mobility ~\cite{xiang2020sapien}
    \item The definition includes six primitive actions that are pose-aware: pre-grasp, grasp, pre-place, and place, as well as manipulation of drawers and manipulation of doors. Based on object pose, these actions enable the execution of pose-related operations and the rapid generation of demos along with their corresponding primitive actions.
    \item 
\end{itemize}













